Self-Supervised Geometry-Aware Encoder for Style-Based 3D GAN Inversion

StyleGAN has achieved great progress in 2D face reconstruction and semantic editing via image inversion and latent editing. While studies over extending 2D StyleGAN to 3D faces have emerged, a corresponding generic 3D GAN inversion framework is still missing, limiting the applications of 3D face reconstruction and semantic editing. In this paper, we study the challenging problem of 3D GAN inversion where a latent code is predicted given a single face image to faithfully recover its 3D shapes and detailed textures. The problem is ill-posed: innumerable compositions of shape and texture could be rendered to the current image. Furthermore, with the limited capacity of a global latent code, 2D inversion methods cannot preserve faithful shape and texture at the same time when applied to 3D models. To solve this problem, we devise an effective self-training scheme to constrain the learning of inversion. The learning is done efficiently without any real-world 2D-3D training pairs but proxy samples generated from a 3D GAN. In addition, apart from a global latent code that captures the coarse shape and texture information, we augment the generation network with a local branch, where pixel-aligned features are added to faithfully reconstruct face details. We further consider a new pipeline to perform 3D view-consistent editing. Extensive experiments show that our method outperforms state-of-the-art inversion methods in both shape and texture reconstruction quality. Code and data will be released.

==> sections/_not_used.tex <==

\heading{GAN Feature Alignment Module}
% Compared with 2D GAN inversion methods which strengthens reconstruction of the input view, 
% 3D GAN inversion is designed for novel view synthesis.
To handle the feature misalignment issue caused by semantic editing~\eg pose and expressions,
2D GAN inversion method~\cite{wang2021HFGI,another} propose to introduce a basic 2D alignment module.
% 
This 2D alignment module takes in the low resolution edited image and original residual map and directly output the aligned residual map.
% 
However, we observe in the experiment that this basic design is both slow and inevitably lead to information loss~\missref in semantic editing.
% 
Inspired by recent study over GAN-based dense correspondences~\misscite,
we propose to directly retrofit the generator feature maps corresponding to the initial image and the edited image as the network input,
and estimate a 2D dense correspondence field $\omega_{est}$ lying in the interval $[-1,1]$ \yslan{re-write the notation range}.
% 
We name the matching module as \GCNICKNAME{}, which stands for GAN Geometry Correspondence Network.
% 
 
Specifically, given a misaligned pair of $\{\hat{\image}, \hat{\image}_{edit}\}$ where $\hat{\image}$ is the reconstructed image and $\hat{\image}_{edit}$ is the edited image,
we retrieve their corresponding generator feature maps $F(\hat{\image})$ and $F(\hat{\image}_{edit})$ and calculate the correspondence field as
% 
\begin{equation}
\label{eq:correspondence}
\GCNICKNAME{}(F(\hat{\image}), F(\hat{\image}_{edit}) = \omega_{est}
\end{equation}
% 
where $F({\image}) \in \gR^{K*H*W*256}$ and we choose $K=4$ here.
The aligned novel view residual feature is warped from the source residual $\hat{\Delta}_{edit}=\hat{\Delta}(\omega_{est})$.

We argue two advantages over this design.
First, since the off-the-shelf generator features directly serve as the network input, 
the heavy image encoder used in the alignment module could be deprecated which significantly improves the inference speed.
Second, our matching model outputs the correspondence field rather than the warped result,
which alleviate extra information loss during the model transformation.
% 
Please refer to the experiments section for more implementation details.
\yslan{compare the inference speed and accuracy; qualitative results.}

Note that unlike previous method~\cite{wang2021HFGI} our alignment module do not need to address the feature misalignment due to pose variations,
since view-consistent 3D features could be directly retrieved via~\ref{eq:local_global_rendering_feat}.

==> sections/discussions.tex <==
\subsection{Limitations and future work}

Limitations:
The 3D shapes of the objects discussed in this paper can still be encoded with a single latent code.

Future work:
geometry side:
3D shapes with large variations such as human.
more complex, adopt local features to predict the geometry along with the global features.

texture side:
currently we only adopt a basic 2D hour-glass encoder to restoring the missing 3D information form the naive GAN inversion,
a more geometry-aware architecture such as 3D convolution used in cost volume based reconstruction methods~\misscite would likely to further improve the reconstruction performance on the novel views.

training side:
currently we need an extra 2D alignment module to assist the editing though lite, still introduces extra computational cost.
In the future work, we aim to find ways to remove this module without sacrificing the reconstruction ability,
and propose an end-to-end training strategy.

Overall,
we believe this work opens a new line of research direction and could serve as a guidance for future works beyond 3D GAN inversion, 
also few-shot 3D reconstructions and 3D-aware learning from 2D images, etc. 

\yslan{contribute: the merits of both priors.}

\yslan{out method could be easily extended to multi-view input.}


and takes a step towards expected 3D GAN inversion.


\heading{Limitations}
disadvantages:
slow sampling.
